ScaleAcross Explorer: Exploring Communication Optimization for Scale-Across AI Model Training

The rapid scaling of large language model training requires distributing GPU resources across multiple data center buildings and regions. We refer to such paradigm as "scale-across" training. As infrastructure expands, the system design space becomes increasingly intricate, encompassing new model architectures, hardware heterogeneity, and evolving communication patterns. Drawing from Meta's production experience, we highlight the complexities of deploying training jobs across a few data centers housing hundreds of thousands of GPUs. To accelerate exploration of the large design space and to enable efficient training for frontier model development, we conduct in-depth characterization of three key design dimensions: parallelism placement, parallelism scheduling, and network layer technologies. We then propose ScaleAcross Explorer, an optimizer that considers the interplay of design dimensions and holistically optimizes scale-across training. Testbed experiments and simulations demonstrate up to 64.62% training speedups over production configuration and up to 37.59% training speedups over the state-of-the-art baseline across a wide range of design points.

==> sections/exploration_settings.tex <==
\section{Scale Across Testbed}
\label{eval:settings}
\minghao{Should reach section 3 around page 3 to 4, needs trimming the above sections.}
To evaluate how production-ready optimization knobs perform in low-bandwidth, high-latency scaling-across training, we conduct network emulation and simulation experiments. This section details our workload configurations, network settings, and experimental baselines.
% \minghao{first list all questions we want to answer. Then start with which questions are we answering with each tool. and that resources and setting for answering each question.}

\subsection{Exploration Overview}
\textbf{Parallelism Placement.}
We first investigate the impact of switching parallelism order. We use {\{Parallelism\}-out} to represent the parallelism placement where \{Parallelism\} is the outermost. Specifically, PP-out refers to PP as the outermost parallelism and DP-out refers to DP as the outermost parallelism. Figure~\ref{fig:dp_out_setting} and ~\ref{fig:pp_out_setting} give the visualization of the DP-out and PP-out setting in emulations. As mentioned in Section~\ref{background:experience_100K}, only DP and PP are being considered as candidates for spanning across buildings. We assume that TP and CP are intra-building and follow the common order that TP is the innermost and CP is the second to the innermost.

\textbf{Parallelism Scheduling.} Both DP-out and PP-out benefit from communication scheduling optimizations. For DP-out, HSDP enables hierarchical gradient synchronization by grouping model replicas. For PP-out, pipeline scheduling and model chunk interleaving help mitigate the high point-to-point communication costs in scale-across training.

\textbf{Network Technology.} As network distance increases, reliability issues become more prevalent. We analyze how link latency, ranging from 10 to 1000~$\mu$s, affects loss recovery and influences the effectiveness of load balancing and congestion control mechanisms.

\subsection{Testbed and Simulation Settings}
\label{method_testbed_simulation}

\begin{table}[t]
\begin{tabular}{|p{0.8cm}|p{0.5cm}|p{0.5cm}|>{\raggedright\arraybackslash}p{1.8cm}|>{\raggedright\arraybackslash}p{1.5cm}|>{\raggedright\arraybackslash}p{1.35cm}|}
\hline
 Model Name & Mbs, Gbs & Seq. Len & TP-CP-EP-PP-DP & Model chunk size & \# Experts \\ \hline
 40B-MoE & 1, 64 & 8K & 4-1-16-2-16 & 2 layer & 16-128\\ \hline
 17B-Dense & 4, 176 & 8K & 8-1-NA-2-4 & 1 layer & NA \\ \hline
  % 17B-MoE & 2 & 176 & 8K & 8 & 2 & 2 & 4 & 1 layer \\ \hline
 % 14.7B & 1 & 256 & 4K & 8 & 1 & 2 & 4 & 2  \\ \hline
 % 2T & 1 & 1536 & 32K & 16 & 4 & 32 & 12 & 1\\ \hline

\end{tabular}
\caption{Configuration of workloads used in testbed experiments and in the emulation. MBS stands for ``MicroBatch Size'' and ``GBS'' stands for ``Global Batch Size''. \minghao{simply labels to "MoE", "dense", "testbed", "simulation"}}
\label{table:workload_configs}
\end{table}

We use testbed experiments to systematically characterize the impact of parallelism placement and scheduling. The production testbed we evaluate on is equipped with tools capable of increasing bandwidth oversubscription ratios by disabling links, and enables reconfiguring cluster distances through optical systems. Our study covers bandwidth oversubscription ratios of 1:1, 1:4, 1:8, and 1:16, encompassing all scenarios described in Table~\ref{table:cross_layers}. The default oversubscription ratio is 1:4 unless specified otherwise. For parallelism scheduling, we evaluate FSDP and HSDP with hierarchical aggregation, as well as the effects of different pipeline schedules using DoraPP and Interleaved ZBV. To ensure that the emulation takeaways apply to much larger scale production settings, we configure the workload to use model architecture similar to production training jobs. The detailed workload configurations are listed in Table~\ref{table:workload_configs}. 

Because the testbed is shared among multiple users, we prioritize experiments with Mixture-of-Experts (MoE) models, which reflects the current trend in model architecture design. For dense model experiments, we utilize a dedicated testbed consisting of 64 NVIDIA H100 GPUs hosted by our research cluster (see Appedix~\ref{app:method_emulator} for detailed description).

\minghao{cite Ying's upcoming NSDI paper. NSDI official website hasn't updated yet with Fall acceptances.}
% \minlan{moved from intro. Discuss why we need simulation here. Not about the problem of emulation, but saying positively on the new aspects simulation brings: we need scale and network simuation }
We cover parallelism placement, communication pattern, and pipeline schedules with the testbed emulations. To fully characterize the optimization space---including the effects of link latency, packet loss rate, and network protocol design---and to enable large-scale evaluation of cross-building network impacts, we employ an in-house packet-level network simulator. 
% This simulator provides a precise modeling of the end-to-end traversal of individual data packets, capturing the behavior of network interface cards (NICs) and switches. It also supports the implementation of custom load balancing and congestion control protocols. 
Simulations are configured using model architectures and workload settings mirroring the 100K GPUs training job we discussed in Section~\ref{background:experience_100K}. We simulate multiple data center buildings and cover 1:1, default, and 2$\times$ and 4$\times$ the default oversubscription ratios (``default ratio'' is based on that of an internal multi-building region), as well as link latencies of 10, 25, 50, 100, and 1000 $\mu$s, with 50 $\mu$s being the default. The default topology is designated as ``Topology A1'' in the later text. To demonstrate the generalizability of our findings, we further simulate multiple topology variants (configuration in Table~\ref{table:topology_configs}). Simulation details are in Appendix~\ref{app:method_simulator}.


==> sections/implementation.tex <==
\section{Implementation}
\label{implementation}
\minlan{Shrink and merge into sec 3}
\subsection{Emulator}
Due to the lack of root access, we have to emulate bandwidth oversubscription between buildings with user space tools. We achieve so by developing a custom NCCL plugin built on top of the original AWS OFI NCCL plugin, which enables NVIDIA's NCCL based applications to use the AWS Elastic Fabric Adapter (EFA). Based on NCCL logs, each server provides 32 available EFA interfaces in total, with four interfaces allocated per GPU. To emulate bandwidth oversubscription on cross-building networks, we exchange rank IDs during communicator initialization and restrict communicators between ranks in different logical buildings to only a subset of the available EFA interfaces.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{sections/old_materials/workload_scaling}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Simulator}
Our simulation leverages an in-house, production-grade network simulator that takes a detailed workload specification describing the computation and communication operations, along with their dependencies, as input. It then models the end-to-end traversal of individual data packets from source GPUs to destination GPUs, accurately capturing the behavior of network interface cards (NICs) and switches. It also supports the implementation of custom load balancing and congestion control protocols.




